Improving Visual Prompt Tuning by Gaussian Neighborhood Minimization for Long-Tailed Visual Recognition

Long-tail learning has garnered widespread attention and achieved significant progress in recent times. However, even with pre-trained prior knowledge, models still exhibit weaker generalization performance on tail classes. The promising Sharpness-Aware Minimization (SAM) can effectively improve the generalization capability of models by seeking out flat minima in the loss landscape, which, however, comes at the cost of doubling the computational time. Since the update rule of SAM necessitates two consecutive (non-parallelizable) forward and backpropagation at each step. To address this issue, we propose a novel method called Random SAM prompt tuning (RSAM-PT) to improve the model generalization, requiring only one-step gradient computation at each step. Specifically, we search for the gradient descent direction within a random neighborhood of the parameters during each gradient update. To amplify the impact of tail-class samples and avoid overfitting, we employ the deferred re-weight scheme to increase the significance of tail-class samples. The classification accuracy of long-tailed data can be significantly improved by the proposed RSAM-PT, particularly for tail classes. RSAM-PT achieves the state-of-the-art performance of 90.3\%, 76.5\%, and 50.1\% on benchmark datasets CIFAR100-LT (IF 100), iNaturalist 2018, and Places-LT, respectively. The source code is temporarily available at https://github.com/Keke921/GNM-PT.

==> tab/CIFAR_RES.tex <==
\begin{table}[t]
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 \centering  % 显示位置为中间
 \caption{Comparison results on CIFAR100-LT w.r.t top-1 classification accuracy (\%).} %
 \label{tab:cifar_results}
 %\vspace{-3pt}
 %\setlength{\tabcolsep}{10pt}
 \resizebox{1.\linewidth}{!}
 %\renewcommand{\arraystretch}{0.95}
  {\begin{threeparttable} %\small
  \begin{tabular}{|c |c | c| c c c c|}
  \hline 
  Method & Year  & Backbone  &200 &100 &50 & 10 \\
  \hline 
  \multicolumn{7}{|c|}{DNN-based model} \\
  \hline 
  BBN~\cite{bbn20} &2020 & ResNet32 & 37.2 & 42.6 & 47.0 & 59.1\\
  RIDE~\cite{WangXD21RIDE}  &2021  & ResNet32 & 45.8 & 50.4 & 55.0 & -\\ 
  MisLAS~\cite{mislas21} & 2021   &ResNet32 &43.5 &47.0 &52.3& 63.2 \\
  BCL~\cite{Zhu2022CVPR} & 2022  &ResNet32 & - & 51.9 & 56.6 & 64.9 \\ 
  GCL~\cite{LiMK2022GCL} & 2022  &ResNet32 & 44.8 & 48.6 & 53.6 & -\\
  NCL~\cite{liJ2022nested} & 2022  &ResNet32 & - & 54.2 & 58.2 & -\\
  GPaCo~\cite{cui2023Gpaco} & 2023  &ResNet32 & - & 52.3 & 56.4 & 65.4\\
  SHIKE~\cite{Jin2023shike} & 2023  & ResNet32 & - & 56.3 & 59.8 & -\\
  \hdashline 
    \multicolumn{7}{|c|}{DNN-based model with SAM} \\
  \hdashline 
  CCSAM~\cite{zhou2023class} & 2023  & ResNet32 & 45.7 & 50.8 & 53.9 & - \\
  ImbSAM~\cite{zhou2023imbsam} & 2023 & ResNet32 & - & 54.8 & 59.3 & 59.7 \\
  \hline
    \multicolumn{7}{|c|}{Attention-based model} \\
  \hline
  VPT~\cite{jia2022visual}  &2022  & ViT-B/16 & 72.8 & 81.0 & 84.8 & 89.6\\
  LiVT~\cite{Xu2023Learning}  &2023 & ViT-B/16 & - & 58.2 & - & 69.2 \\ 
  LPT~\cite{Dong23LPT}  &2023 & ViT-B/16 & \textbf{87.9} & \textbf{89.1} & \textbf{90.0} & \textbf{91.0}\\ 
  \hdashline 
  GNM-PT &  Ours  & ViT-B/16 & \underline{\textbf{89.2}} & \underline{\textbf{90.3}} & \underline{\textbf{91.2}} & \underline{\textbf{91.8}} \\ 
  \hline
  % \bottomrule
 \end{tabular}
    \begin{tablenotes}
    %\footnotesize
    \item \textbf{Note}: The best and the second-best results are shown in \underline{\textbf{underline bold}} and \textbf{bold}, respectively.
    %\item \textbf{DR}, decoupling representation. \textbf{MU}, MixUp. \textbf{BSCE}, balanced softmax cross entropy loss.
    \end{tablenotes}
 \end{threeparttable}
 }
%\vspace{-9pt}
\end{table}

==> tab/ComSam_tab_fig.tex <==

\begin{figure}[t]
\begin{minipage}{0.55\textwidth}
\centering
    \includegraphics[width=1.\textwidth]{Styles/fig/histogram/his_gcl_ce.pdf} 
    \vspace{-12pt}
    \figcaption{Effectiveness comparison of different classes.} %The results of GCL are combined with DRW.
    \label{fig:histogram}
\end{minipage}
\hspace{3pt}
\begin{minipage}[h]{0.43\linewidth}
\vspace{-12pt}
 \tabcaption{Comparison between SAM and the proposed GNM. NET represents Native Execution Time.} % on CIFAR-100-LT with imbalance factor of 100.
 \vspace{6pt}
 \label{tab:com_sam}
 %\setlength{\tabcolsep}{10pt}
 \resizebox{1.\textwidth}{!}
 %\renewcommand{\arraystretch}{0.9}
  {
  \begin{tabular}{ l | c  c }
  \hlinew{1pt}
  Method & Acc. (\%) & NET (s) \\ 
  \hline
  CE    & 81.02 &  39.78\\
  CE+SAM & 82.48 & 72.51\\
  \rowcolor{mygray}
  CE+GNM & \textbf{82.50} & 40.16 ({\color{purple}{$\downarrow$ 44.61\%}} )\\ 
  \cdashline{1-3} %\hdashline
  GCL+DRW  & 89.58 & 40.00 \\
  GCL+DRW+SAM & 89.69 & 74.36   \\
  \rowcolor{mygray}
  GCL+DRW+GNM & \textbf{90.28} & 41.87 ({\color{purple}{$\downarrow$ 43.69\%}} )\\
  \hlinew{1pt}
 \end{tabular}
 }
\end{minipage}
\end{figure}

==> tab/IMG_RES.tex <==

\begin{table}[t]
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 \centering  % 显示位置为中间
 \caption{Comparison results on ImageNet-LT.} \label{tab:img} % \wrt Top-1 accuracy (\%)
 %\vspace{-3pt}
 %\setlength{\tabcolsep}{6pt}
 \resizebox{1.\linewidth}{!}
 %\renewcommand{\arraystretch}{1.1}
  {\begin{threeparttable}
\begin{tabular}{|c |c |c c c |c|}  
  \hline
  Method & Year &Head &Med &Tail & Overall \\
  \hline
    \multicolumn{6}{|c|}{Backbone: ViT-B/16}\\ %
  \hline 
    \multicolumn{6}{|c|}{With supplementary data} \\
  \hline
    VL-LTR~\cite{tian2022vl} &2022  & 84.5 & 74.6 & 59.3 & 77.2$^\dag$ \\ 
    GML~\cite{SuhS23GML} &2023  & - & - & - & \textbf{78.0}$^\dag$\\ 
  \hline
    \multicolumn{6}{|c|}{Visual-only} \\
  \hline 
  BALLAD ~\cite{ma2021simple}  &2021  & 79.1 & 74.5 & 69.8 & 75.7 \\ 
  VPT~\cite{jia2022visual}  &2022  & 79.5 & 76.5 & 72.8 & \textbf{77.2} \\
  Decoder ~\cite{wang2023exploring} &2023  & - & - & - & 73.2 \\ 
  \hdashline
  GNM-PT & Ours&80.6 & 81.1 & 78.2 & \underline{\textbf{80.4}}\\ 
  \hline
  % \bottomrule
 \end{tabular}
    \begin{tablenotes}
    %\footnotesize
    \item \textbf{Note}: The same as \cref{tab:inat}.
    \end{tablenotes}
 \end{threeparttable}
 }
%\vspace{-6pt}
\end{table}



==> tab/PLA_RES.tex <==

\begin{table}[t]
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 \centering  % 显示位置为中间
 \caption{Comparison results on Places-LT.} \label{tab:pla} % w.r.t top-1 classification accuracy (\%)
 %\vspace{-3pt}
 %\setlength{\tabcolsep}{6pt}
 \resizebox{1.\linewidth}{!}
 %\renewcommand{\arraystretch}{1.1}
  {\begin{threeparttable}
  \begin{tabular}{|c |c |c |c c c |c|}  
  \hline 
  Method & Year & Backbone & Head & Med &Tail & Overall \\
  \hline 
    \multicolumn{7}{|c|}{DNN-based model} \\
  \hline     
  LWS~\cite{decouple20} &2020 & ResNet152 & 40.6 & 39.1 & 28.6 & 37.6\\
  RIDE~\cite{WangXD21RIDE}  &2021  & ResNet152 & 44.4 & 40.6 & 33.0 & 40.4 \\ 
  MisLAS~\cite{mislas21} & 2021   &ResNet152 & 39.6 & 43.3 & 36.1 & 40.4 \\
  GCL~\cite{LiMK2022GCL} & 2022  &ResNet152 & 38.6 & 42.6 & 38.4 & 40.3 \\
  NCL~\cite{liJ2022nested} & 2022  &ResNet152 & - & - & - & 41.8 \\
  GPaCo~\cite{cui2023Gpaco} & 2023  &ResNet152 & 39.5 & 47.2 & 33.0 & 41.7\\
  SHIKE~\cite{Jin2023shike} & 2023  & ResNet152 & 43.6 & 39.2 & 44.8 & 41.9 \\
  \hdashline 
    \multicolumn{7}{|c|}{DNN-based model with SAM} \\
  \hdashline   
  CCSAM~\cite{zhou2023class} & 2023  & ResNet152 & 41.2 & 42.1 & 36.4  & 40.6 \\ 
  \hline
    \multicolumn{7}{|c|}{Attention-based model} \\
  \hline
    \multicolumn{7}{|c|}{With supplementary data} \\
  \hdashline 
    VL-LTR~\cite{tian2022vl} &2022 & ViT-B/16   & 54.2 & 48.5 & 42.0 & \underline{\textbf{50.1}}$^\dag$ \\ 
    RAC~\cite{Long2022RAC} & 2022  & ViT-B/16   & 48.7 & 48.3 & 41.8 & 47.2$^\dag$\\ 
  \hdashline 
    \multicolumn{7}{|c|}{Visual-only} \\
  \hdashline  
  Decoder ~\cite{wang2023exploring} &2023  &ViT-B/16   & - & - & - & 46.8 \\ 
  LPT~\cite{Dong23LPT}  &2023 & ViT-B/16 & 54.2 & 48.5 & 42.0 & \underline{\textbf{50.1}} \\ 
  LiVT~\cite{Xu2023Learning}  &2023 & ViT-B/16 & 48.1 & 40.6 & 27.5 & 40.8 \\ 
  \hdashline
  GNM-PT  &  Ours & ViT-B/16    & 46.6 & 53.3 & 49.4 & \underline{\textbf{50.1}} \\ 
  GNM-PT$^\star$  &  Ours & ViT-B/16    & 48.6 & 52.1 & 47.9 & \textbf{50.0} \\ 
  \hline
  % \bottomrule
 \end{tabular}
    \begin{tablenotes}
    %\footnotesize
    \item \textbf{Note}: %Med, medium split.
    The same as \cref{tab:inat}.
    %\item $\star$ represents the result obtained without DRW.
    \end{tablenotes}
 \end{threeparttable}
 }
\end{table}

==> tab/PLA_RES2.tex <==
\begin{table}[t]
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 \centering  % 显示位置为中间
 \caption{Acc. (\%) comparison on Places-LT.} \label{tab:pla} % w.r.t top-1 classification accuracy (\%)
 %\vspace{3pt}
 %\setlength{\tabcolsep}{6pt}
 \resizebox{0.7\linewidth}{!}
 %\renewcommand{\arraystretch}{1.1}
  {\begin{threeparttable}
  \begin{tabular}{|c |c c c |c|}  
  \hline 
  Method  & Head & Med &Tail & Overall \\
  \hline 
    \multicolumn{5}{|c|}{DNN-based model (Backbone: ResNet152)} \\
  \hline     
  LWS~\cite{decouple20}   & 40.6 & 39.1 & 28.6 & 37.6\\
  RIDE~\cite{WangXD21RIDE}   & 44.4 & 40.6 & 33.0 & 40.4 \\ 
  MisLAS~\cite{mislas21}  & 39.6 & 43.3 & 36.1 & 40.4 \\
  GCL~\cite{LiMK2022GCL}  & 38.6 & 42.6 & 38.4 & 40.3 \\
  NCL~\cite{liJ2022nested}  & - & - & - & 41.8 \\
  GPaCo~\cite{cui2023Gpaco}  & 39.5 & 47.2 & 33.0 & 41.7\\
  SHIKE~\cite{Jin2023shike}  & 43.6 & 39.2 & 44.8 & 41.9 \\
  \hdashline 
    \multicolumn{5}{|c|}{DNN-based model with SAM} \\
  \hdashline   
  CCSAM~\cite{zhou2023class}  & 41.2 & 42.1 & 36.4  & 40.6 \\ 
  \hline
    \multicolumn{5}{|c|}{MHSA-based model  (Backbone: ViT-B/16)} \\
  \hline
    \multicolumn{5}{|c|}{Supplementary with linguistic data} \\
  \hdashline 
    VL-LTR~\cite{tian2022vl}   & 54.2 & 48.5 & 42.0 & \underline{\textbf{50.1}}$^\dag$ \\ 
    RAC~\cite{Long2022RAC}  & 48.7 & 48.3 & 41.8 & 47.2$^\dag$\\ 
  \hdashline 
    \multicolumn{5}{|c|}{Visual-only} \\
  \hdashline  
  Decoder ~\cite{wang2023exploring}   & - & - & - & 46.8 \\ 
  LPT~\cite{Dong23LPT}   & 54.2 & 48.5 & 42.0 & \underline{\textbf{50.1}} \\ 
  LiVT~\cite{Xu2023Learning}   & 48.1 & 40.6 & 27.5 & 40.8 \\ 
  \hdashline
  GNM-PT     & 46.6 & 53.3 & 49.4 & \underline{\textbf{50.1}} \\ 
  GNM-PT$^\star$   & 48.6 & 52.1 & 47.9 & \textbf{50.0} \\ 
  \hline
  % \bottomrule
 \end{tabular}
    \begin{tablenotes}
    %\footnotesize
    \item \textbf{Note}: %Med, medium split.
    The same as \cref{tab:inat}.
    %\item $\star$ represents the result obtained without DRW.
    \end{tablenotes}
 \end{threeparttable}
 }
 %\vspace{-6pt}
\end{table}

==> tab/iNat_RES.tex <==
\begin{table}[t]
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 \centering  % 显示位置为中间
 \caption{Comparison results on iNat.} \label{tab:inat} % \wrt Top-1 accuracy (\%)
 %\vspace{-3pt}
 %\setlength{\tabcolsep}{6pt}
 \resizebox{1\linewidth}{!}
 %\renewcommand{\arraystretch}{1.1}
  {\begin{threeparttable}
  \begin{tabular}{|c |c |c |c c c |c|}  
  \hline 
  Method & Year & Backbone & Head & Med &Tail & Overall \\
  \hline 
    \multicolumn{7}{|c|}{DNN-based model} \\
  \hline     
  LWS~\cite{decouple20} &2020 & ResNet50 & 72.9 & 71.2 & 69.2 & 70.5\\
  RIDE~\cite{WangXD21RIDE}  &2021  & ResNet50 & 76.5 & 74.2 & 70.5 & 72.8 \\ 
  MisLAS~\cite{mislas21} & 2021   &ResNet50 & 73.2 & 72.4 &70.4 & 71.6 \\
  BCL~\cite{Zhu2022CVPR} & 2022  &ResNet50 & - & - & - & 71.8 \\ 
  GCL~\cite{LiMK2022GCL} & 2022  &ResNet50 & - & - &- & 72.0\\
  NCL~\cite{liJ2022nested} & 2022  &ResNet50 & 72.7 & 75.6 & 74.5 & 74.9 \\
  GPaCo~\cite{cui2023Gpaco} & 2023  &ResNet50 & - & - & - & 75.4\\
  SHIKE~\cite{Jin2023shike} & 2023  & ResNet50 & - & - & - & 75.4 \\
  \hdashline 
    \multicolumn{7}{|c|}{DNN-based model with SAM} \\
  \hdashline 
   LDAM+SAM~\cite{rangwani2022escaping} & 2022 & ResNet50 & 64.1 & 70.5 & 71.2 & 70.1 \\   %{\small LDAM~\cite{Kaidi2019}+SAM~\cite{rangwani2022escaping}}  
  CCSAM~\cite{zhou2023class} & 2023  & ResNet50 & 65.4 & 70.9 & 72.2  & 70.9 \\ 
  ImbSAM~\cite{zhou2023imbsam} & 2023 & ResNet50 & 68.2 & 72.5 & 72.9 & 71.1\\
  \hline
    \multicolumn{7}{|c|}{Attention-based model} \\
  \hline
    \multicolumn{7}{|c|}{With supplementary data} \\
  \hdashline 
    VL-LTR~\cite{tian2022vl} &2022 & ViT-B/16   & - & - & - & \textbf{76.8}$^\dag$ \\ 
    RAC~\cite{Long2022RAC} & 2022  & ViT-B/16   & 75.9 & 80.5 & 81.1 & \underline{\textbf{80.2}}$^\dag$ \\ 
  \hdashline 
    \multicolumn{7}{|c|}{Visual-only} \\
  \hdashline  
  Decoder ~\cite{wang2023exploring} &2023  &ViT-B/16   & - & - & - & 59.2 \\ 
  LPT~\cite{Dong23LPT}  &2023 & ViT-B/16 & - & - & 79.3 & 76.1 \\ 
  LiVT~\cite{Xu2023Learning}  &2023 & ViT-B/16 & 78.9 & 76.5 & 74.8 & 76.1 \\ 
  \hdashline
  GNM-PT   & Ours & ViT-B/16    &61.5 & 77.1 & 79.3 & \underline{\textbf{76.5}} \\ 
  GNM-PT$^\star$  & Ours & ViT-B/16    &76.3& 77.6 & 75.0 & \textbf{76.3} \\ 
  \hline
  % \bottomrule
 \end{tabular}
    \begin{tablenotes}
    %\footnotesize
    \item  %Med, medium split.
    \textbf{Note}: The best and the second-best results are shown in \underline{\textbf{underline bold}} and \textbf{bold}, respectively.
    \item Med: is short for Medium classes.
    \item $^\dag$: The results are obtained with the assistance of textual data.
    %, we also emphasize the best and second-bast results from others based solely on visual data.
    \item $\star$ represents the result obtained without DRW.    
    \end{tablenotes}
 \end{threeparttable}
 }
%\vspace{-9pt}
\end{table}

==> tab/iNat_RES2.tex <==
\begin{table}[t]
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
 \centering  % 显示位置为中间
 \caption{Acc. (\%) comparison on iNat.} \label{tab:inat} % \wrt Top-1 accuracy (\%)
 %\vspace{3pt}
 %\setlength{\tabcolsep}{6pt}
 \resizebox{0.7\linewidth}{!}
 %\renewcommand{\arraystretch}{1.1}
  {\begin{threeparttable}
  \begin{tabular}{|c |c c c |c|}  
  \hline 
   Method & Head & Med & Tail & Overall \\
  \hline 
    \multicolumn{5}{|c|}{DNN-based model (Backbone: ResNet50)} \\
  \hline     
  LWS~\cite{decouple20}    & 72.9 & 71.2 & 69.2 & 70.5\\
  RIDE~\cite{WangXD21RIDE}   & 76.5 & 74.2 & 70.5 & 72.8 \\ 
  MisLAS~\cite{mislas21}  & 73.2 & 72.4 &70.4 & 71.6 \\
  BCL~\cite{Zhu2022CVPR}  & - & - & - & 71.8 \\ 
  GCL~\cite{LiMK2022GCL}  & - & - &- & 72.0\\
  NCL~\cite{liJ2022nested}  & 72.7 & 75.6 & 74.5 & 74.9 \\
  GPaCo~\cite{cui2023Gpaco} & - & - & - & 75.4\\
  SHIKE~\cite{Jin2023shike}  & - & - & - & 75.4 \\
  \hdashline 
    \multicolumn{5}{|c|}{DNN-based model with SAM  } \\
  \hdashline 
   {\small LDAM+SAM~\cite{rangwani2022escaping}} & 64.1 & 70.5 & 71.2 & 70.1 \\   %{\small LDAM~\cite{Kaidi2019}+SAM~\cite{rangwani2022escaping}}  
  CCSAM~\cite{zhou2023class} & 65.4 & 70.9 & 72.2  & 70.9 \\ 
  ImbSAM~\cite{zhou2023imbsam} & 68.2 & 72.5 & 72.9 & 71.1\\
  \hline
    \multicolumn{5}{|c|}{MHSA-based model (Backbone: ViT-B/16) } \\
  \hline
    \multicolumn{5}{|c|}{Supplementary with linguistic data} \\
  \hdashline 
    VL-LTR~\cite{tian2022vl} & - & - & - & \textbf{76.8}$^\dag$ \\ 
    RAC~\cite{Long2022RAC}  & 75.9 & 80.5 & 81.1 & \underline{\textbf{80.2}}$^\dag$ \\ 
  \hdashline 
    \multicolumn{5}{|c|}{Visual-only} \\
  \hdashline  
  Decoder~\cite{wang2023exploring} & - & - & - & 59.2 \\ 
  LPT~\cite{Dong23LPT} & - & - & 79.3 & 76.1 \\ 
  LiVT~\cite{Xu2023Learning}  & 78.9 & 76.5 & 74.8 & 76.1 \\ 
  \hdashline
  GNM-PT &61.5 & 77.1 & 79.3 & \underline{\textbf{76.5}} \\ 
  GNM-PT$^\star$  &76.3& 77.6 & 75.0 & \textbf{76.3} \\ 
  \hline
  % \bottomrule
 \end{tabular}
    \begin{tablenotes}
    %\footnotesize
    \item  %Med, medium split.
    \textbf{Note}: The best and the second-best results are shown in \underline{\textbf{underline bold}} and \textbf{bold}, respectively.
    \item Med: is short for Medium classes.
    \item $^\dag$: The results are obtained with the assistance of textual data.
    %, we also emphasize the best and second-bast results from others based solely on visual data.
    \item $\star$ represents the result obtained without DRW.    
    \end{tablenotes}
 \end{threeparttable}
 }
\end{table}

==> tab/rebuttal_Com_strategy1.tex <==
\begin{table}[!h]
 \centering  % 显示位置为中间
 \tabcaption{Optimization strategy comparison (with stage1 only).} %
 \label{tab:rbu_wost2}
 \setlength{\tabcolsep}{5pt}
 \resizebox{0.55\linewidth}{!}
 %\renewcommand{\arraystretch}{1.2}
 {%\begin{threeparttable}
      %\small
      \begin{tabular}{l |c c c c c }  
          \hlinew{1pt}
          Method  &  Head &	Med	& Tail &All & NET(s) \\
          \hline
          Base & 92.86 & 88.94 & 79.28 & 87.76 & \textbf{40.32} \\
          Base + CCSAM & 92.81 & 88.31 & 79.31 & 87.84 & 80.47 \\
          Base + ImbSAM & 92.92 & 88.43 & \textbf{84.00} & \textbf{89.02} & 88.97 \\
          \rowcolor{mygray}
          Base + GNM-PT & \textbf{93.67} & \textbf{89.03} & 81.10 & 88.46 & 42.77 \\
          \hlinew{1pt}
        \end{tabular}
        %\begin{tablenotes}
            %\footnotesize
            %\item \textbf{Note}: NET represents native execution time.
            %\item \textbf{DR}, decoupling representation. \textbf{MU}, MixUp. \textbf{BSCE}, balanced softmax cross entropy loss.
        %\end{tablenotes}
%\end{threeparttable}
}
\end{table}



==> tab/rebuttal_Com_strategy2.tex <==
\begin{table}[!h]
  \centering  % 显示位置为中间
 \tabcaption{Optimization strategy comparison (with stage2).} %
 \label{tab:rbu_wst2}
 \setlength{\tabcolsep}{5pt}
 \resizebox{0.55\linewidth}{!}
 %\renewcommand{\arraystretch}{1.2}
 {\begin{threeparttable}
      %\small
      \begin{tabular}{l |c c c c c }  
          \hlinew{1pt}
          Method  &  Head &	Med	& Tail &All \\
          \hline
          LPT & - & - & - & 89.10 \\
          \cdashline{1-5} 
          Base & 90.08 ($\downarrow$ 2.78) & 89.60 & 88.14 & 89.40 \\
          Base + CCSAM & 90.47 ($\downarrow$ 2.34) & 89.63 & 88.03 & 89.54 \\
          Base + ImbSAM & 91.75 ($\downarrow$ 1.17) & 88.71 & 87.90 & 89.62 \\
          \rowcolor{mygray}
          Base + GNM-PT & \textbf{91.94} ($\downarrow$ 1.73) & \textbf{90.17} & \textbf{88.21} & \textbf{90.28} \\
          \hlinew{1pt}
     \end{tabular}
        \begin{tablenotes}
            %\footnotesize
            \item \textbf{Note}: The listed decreases in Head accuracy (\%) are compared to that in \cref{tab:rbu_wost2}
        \end{tablenotes}
\end{threeparttable}
}
\end{table} 
